Revisiting the definition of rapid intensification of tropical cyclones by clustering the initial intensity and inner-core size

Rapid intensification (RI) of tropical cyclones (TCs) provides a great challenge in operational forecasting and contributes significantly to the development of major TCs. RI is commonly defined as an increase in the maximum sustained surface wind speed beyond a certain threshold within 24 h. The most widely used threshold is 30 kt (15.4 m/s), which was determined statistically. Here we propose a new definition for RI by objectively clustering TCs using the intensification rate, initial intensity, and radius of the maximum wind speed. A group of 770 samples is separated at a threshold of 45 kt (23.2 m/s). The threshold is 40 kt (20.6 m/s) for the western North Atlantic, where TC size measurements are more reliable. Monte Carlo experiments demonstrate that the proposed threshold is robust even considering the uncertainty in RMW of as high as 30 km. We show that, when a TC undergoes RI, its maximum wind speed is approximately 60+/-15 kt (30.9+/-7.7 m/s) and the radius of the maximum wind speed is 45+/-20 km. The new threshold outperforms the conventional threshold of 30 kt/24h in (1) describing the bimodal distribution of lifetime maximum intensity, and (2) explaining the annual count of Category 5 TCs. This new definition provides a more physically-based threshold and describes a more reliable representation to the extreme events. Although more comparisons are needed for operational application, it is likely to be desirable for process-based case studies, and could provide a more valuable metric for TC intensification classification and research.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -cd -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk -cd \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -cd -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -cd -lualatex \"$_[0]\"" );
   }
}
